Stingray: Fast Concurrent Transactions Without Consensus

Recent advances have improved the throughput and latency of blockchains by processing transactions accessing different parts of the state concurrently. However, these systems are unable to concurrently process (a) transactions accessing the same state, even if they are (almost) commutative, e.g., payments much smaller than an account's balance, and (b) multi-party transactions, e.g., asset swaps. Moreover, they are slow to recover from contention, requiring once-in-a-day synchronization. We present Stingray, a novel blockchain architecture that addresses these limitations. The key conceptual contributions are a replicated bounded counter that processes (almost) commutative transactions concurrently, and a FastUnlock protocol that uses a fallback consensus protocol for fast contention recovery. We prove Stingray's security in an asynchronous network with Byzantine faults and demonstrate on a global testbed that Stingray achieves 10,000 times the throughput of prior systems for commutative workloads.

==> sections/discussion.tex <==
%

%

\section{Handling Gas Objects}
Typical transactions not only mutate objects but also consume a gas object to spend for the computation. If, however, the transaction is locked then this gas is blocked as well. For this reason \sysname requires a fresh gas-object in order for consensus to process the unlock request.
Specifically together with~\Cref{alg:process-unlock-tx}, the parties should provide a fresh gas object for their request. This gas object is checked for validity along with the check in~\Cref{alg:line:verify-auth} and locked for the unlock transaction in~\Cref{alg:line:block-exec}. When the user collects the no-commit proof in the second step of the protocol, the $2f+1$ collected signatures also serve as a certificate for the gas object. The consensus then checks the validity of the certificate and spends it locally before entering~\Cref{alg:process-unlock-cert}.
Then when consensus executes the transaction three scenarios may happen:

\begin{itemize}
    \item The unlock request is valid and includes a certificate. Then the execution happens as usual and both the gas object for the unlock and the gas object for the execution are consumed.
    \item The unlock requests is valid and comes with a no-op. Then the gas object for unlock is consumed. If there was some locked transaction racing the \fun then the accompanying gas object is potentially blocked. The user can then explicitly unlock that gas object by running \fun.
    \item The unlock request is not processed because a checkpoint certificate already executed a transaction. Then the gas object is still consumed without altering the state of the $\Okey$.
\end{itemize}

%
%

==> sections/mysticeti_commutativity.tex <==
\section{Commutative Transactions on the Mysticeti DAG}


==> sections/mysticeti_fastunlock.tex <==
\section{FastUnlock on the Mysticeti DAG}
